BlockFLA: Accountable Federated Learning via Hybrid Blockchain Architecture

Federated Learning (FL) is a distributed, and decentralized machine learning protocol. By executing FL, a set of agents can jointly train a model without sharing their datasets with each other, or a third-party. This makes FL particularly suitable for settings where data privacy is desired. At the same time, concealing training data gives attackers an opportunity to inject backdoors into the trained model. It has been shown that an attacker can inject backdoors to the trained model during FL, and then can leverage the backdoor to make the model misclassify later. Several works tried to alleviate this threat by designing robust aggregation functions. However, given more sophisticated attacks are developed over time, which by-pass the existing defenses, we approach this problem from a complementary angle in this work. Particularly, we aim to discourage backdoor attacks by detecting, and punishing the attackers, possibly after the end of training phase. To this end, we develop a hybrid blockchain-based FL framework that uses smart contracts to automatically detect, and punish the attackers via monetary penalties. Our framework is general in the sense that, any aggregation function, and any attacker detection algorithm can be plugged into it. We conduct experiments to demonstrate that our framework preserves the communication-efficient nature of FL, and provide empirical results to illustrate that it can successfully penalize attackers by leveraging our novel attacker detection algorithm.

==> threat_model.tex <==
% \section{Threat Model}\label{sec:threat}
% \MS{I didn't understand this section at all, leaving it as it is.}

% The \blockfl system can encounter multiple types of attacks through it's course of execution. One such attack is the trojan based attack which involves the attacker implementing semantic backdoors in the aggregation of parameters. 
% \MK{Where this 2/3rd assumption comes from. How do we address.}
% We assume that at least \sfrac{2}{3}rd of the workers sending the trained model are honest in training the model and sending parameters. \blockfl assures correctness if at least \sfrac{2}{3}rd of the participants are honest. 
% Furthermore, we assume that since the parties have joined the private blockchain and due to its nature of being permissioned, the membership provider of the private chain possess identity details of the workers and confirm the account created and affiliated with the smart contract on the public chain. 

% The second type of attack involves a worker node being blatantly dishonest in the sense that the parameters sent by them during the Federated Averaging execution are different than those sent during the investigation phase. 
% \MK{Again this does not make sense. Please clarify.}
% In this scenario, we can assume the 51\% attack and consider all worker nodes could potentially be malicious in that way. 

% The third type of attack presumes the keys of the worker nodes being compromised thus allowing the attacker to send the model parameters on behalf of the worker node who's keys are compromised. Here, we assume that the attacker could be a participant on the blockchain or they could be an entity not affiliated with the blockchain. 

% \MK{Do we need this assumption? I thought the server runs on the blokchain hence. we do not need trust. Clarify !!!}
% In all the above attacks, we assume that the server node behaves honestly by aggregating parameters correctly and sending the parameters to the correct participants. We also assume that each participant has an account on both the public and private chain and 
% \MK{Again, why do we need this?? Please clarify. We can check that they are the same. cannot we? Please do not know put any unnecessary assumptions.}
% all participants send the same number of parameters to allow efficient aggregation.
